Exceptional supercuspidal representations in small residue characteristic

In this paper, in residue characteristic 2 and 3, we extend the construction of epipelagic representations of Reeder--Yu to produce new supercuspidals of higher depth, building on work of Gastineau. In particular, we produce examples of epipelagic representations that do not arise from the construction of Reeder--Yu.

==> dynkinF.tex <==
%%%%%%%%%%%%%%%% TYPE F4 %%%%%%%%%%%%%%%%%%%%%%%%

\begin{center}

\begin{tikzpicture}[
  scale=1.5,
  vertex/.style={fill=black, circle, inner sep=0pt, minimum size=6pt},
  empty vertex/.style={circle, draw=black, inner sep=0pt, minimum size=6pt},
  every path/.style={thick},
  label style/.style={below=4pt},
]

\coordinate (0) at (0,0);
\coordinate (1) at (1,0);        % alpha_2 center
\coordinate (2) at (2,0);     % alpha_3 to the right
\coordinate (3) at (3,0);
\coordinate (4) at (4,0);

% Nodes with labels
\node[empty vertex] (0) at (0) {};
\node[label style] at (0) {$-\alpha_0$};

\node[vertex] (1) at (1) {};
\node[label style] at (1) {$\alpha_1$};

\node[vertex] (2) at (2) {};
\node[label style] at (2) {$\alpha_2$};

\node[vertex] (3) at (3) {};
\node[label style] at (3) {$\alpha_{3}$};

\node[vertex] (4) at (4) {};
\node[label style] at (4) {$\alpha_{4}$};


% Edges - uniform length ~1 unit

\draw (0) -- (1);
\draw (1) -- (2);
\draw (3) -- (4);        


% Double bond lines close together
\draw (2)++(0,0.04) -- ++(1,0);
\draw (2)++(0,-0.04) -- ++(1,0);

\coordinate (Vmid2) at ($(2)!0.5!(3)$);
\begin{scope}[shift={(Vmid2)}, rotate=0]
  \draw[thick] (0,0.1) -- (0.15,0) -- (0,-0.1);
\end{scope}


\end{tikzpicture}
    
\end{center}
